Optimizing digital spectrometers for radioastronomical observations

The goal of this thesis was to develop a procedure to optimize the mirror suppression, which reduces the dynamic range of the Fast Fourier Transform spectrometers (FFTS), and implement this procedure in the Field Programmable Gate Array (FPGA) of the FFTS. This is achieved by applying a calibration on the complex amplitude spectrum. Modern multi-beam heterodyne receivers are equipped with a large number of independent signal chains, which leads to a complex system that consumes space as well as power and is expensive. To reduce the complexity of the receiver array the intermediate frequency (IF) band is 4-8 GHz, which requires the FFTS to sample this band directly. The input bandwidth of 4 GHz of the current generation of FFTS cannot be sampled with a single analog-digital converter (ADC). To reach that bandwidth, multiple ADCs sample the same signal at different points in time. The method is called \"time interleaved sampling\". The characteristics of the ADCs differ from each other, which leads to mirror signals in the spectrum. These mirror signals can reduce the dynamic range of the spectrometers. Therefore the mismatches must be actively corrected. The current generation of FFTS use a frequency independent calibration, which optimizes the mirror suppression at one fixed frequency. This it is not optimal as some of the mismatches are frequency dependent and their impact increases with frequency. The procedure developed during this thesis work involves three steps. First the mismatches are measured over the frequency band. Then filter coefficients are calculated from these mismatches using a model of a time interleaved ADC. These filter coefficients are then applied to the complex amplitude spectra of the ADCs. The newly implemented calibration improves the mirror suppression up to 20 dB compared to the frequency independent calibration.

==> Makefile <==
# Makefile to run latex, dvips, and pdflatex on a thesis
# Can also run feynmf/feynmp/tikz on files in a directory

THESIS = mythesis
# EXTRACMD = --shell-escape
FEYNDIR = ../feynmf
FEYNFILES = $(wildcard $(FEYNDIR)/*.tex)
TIKZDIR = ../tikz
TIKZFILES = $(wildcard $(TIKZDIR)/*.tex)
ifdef file
FEYNFILES = $(FEYNDIR)/$(file).tex
TIKZFILES = $(TIKZDIR)/$(file).tex
endif
BIBTEX = biber
AWKDIR=..

.PHONY: thesis cover \
	feynmf feynmp tikz \
	cleanthesis cleancover \
	cleanfeynmf cleanfeynmp cleantikz cleanpictpdf \
	cleanblx cleanbbl \
	cleanglo \
	help test

thesis: thesis11

# - in front of bibtex means compilation continues even if there is an error
thesis09: $(THESIS).tex *.tex *.bib
	pdflatex   $(EXTRACMD) $(THESIS)
	-bibtex $(THESIS)
	# makeglossaries $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)
	makeglossaries $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)

thesis11: $(THESIS).tex *.tex *.bib
	pdflatex   $(EXTRACMD) $(THESIS)
	$(BIBTEX)  $(THESIS)
	# makeglossaries $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)
	makeglossaries $(THESIS)
	pdflatex   $(EXTRACMD) $(THESIS)

cover:
	pdflatex   $(EXTRACMD) cover_only
	pdflatex   $(EXTRACMD) cover_only

feynmf:
	make -f ../Makefile FEYNDIR=$(FEYNDIR) FEYNFILES="$(FEYNFILES)" \
	 AWKDIR=$(AWKDIR) feynmf

feynmp:
	make -f ../Makefile FEYNDIR=$(FEYNDIR) FEYNFILES="$(FEYNFILES)" \
	 AWKDIR=$(AWKDIR) feynmp

tikz:
	make -f ../Makefile TIKZDIR=$(TIKZDIR) TIKZFILES="$(TIKZFILES)" tikz

thesis_feynmf:
	feynmf $(THESIS)

cleanall: clean cleanbbl cleanpictpdf

clean: cleanthesis cleancover \
	cleanfeynmf cleanfeynmp cleantikz \
	cleanblx cleanglo

cleanthesis:
	-rm $(THESIS).log $(THESIS).aux $(THESIS).toc
	-rm $(THESIS).lof $(THESIS).lot $(THESIS).out
	-rm $(THESIS).blg $(THESIS).bbl $(THESIS).pdf
	-rm *.aux

cleancover:
	-rm cover_only.log cover_only.aux cover_only.out
	-rm cover_only.pdf

cleanfeynmf:
	-rm *.mf *.tfm *.t1 *.600gf *.600pk *.log
	-rm feynmf_all.* feynmf_files.inp

cleanfeynmp:
	-rm *.1 *.log *.mp *.t1
	-rm feynmf_all.* feynmf_files.inp

cleantikz:
	-rm tikz/*.log tikz/*.aux

cleanpictpdf:
	-rm feynmf/*.pdf
	-rm tikz/*.pdf

cleanblx:
	-rm *-blx.bib
	-rm *.bcf
	-rm *.run.xml

cleanbbl:
	-rm *.bbl

cleanglo:
	-rm *.acn *.acr *.alg
	-rm *.glg *.glo *.gls
	-rm *.ist

help:
	@echo "Possible commands:"
	@echo "new [THESIS=dirname]: Set up a new thesis"
	@echo "thesis: Compile complete thesis (thesis11)"
	@echo "thesis09: Compile complete thesis - texlive 2009 + bibtex"
	@echo "thesis11: Compile complete thesis - texlive >=2011 + biber"
	@echo "feynmf: Run feynmf for all .tex files in $(FEYNDIRNAME)"
	@echo "feynmp: Run feynmp for all .tex files in $(FEYNDIRNAME)"
	@echo "tikz:   Run tikz for all .tex files in $(TIKZDIRNAME)"
	@echo "cleanthesis: Clean up thesis LaTeX output files"
	@echo "cleanfeynmf: Clean up feynmf output files"
	@echo "cleanbbl:    Clean up thesis bbl files"
	@echo "cleanblx:    Clean up thesis biber files"
	@echo "cleantikz:   Clean up tikz output files"
	@echo "cleanglo:    Clean up glossary output files"

test:
	@echo "Thesis $(THESIS)"
	@echo "Feynmf Feynman graphs dir: $(FEYNDIRNAME)"
	@echo "Feynmf Feynman graphs files: $(FEYNFILES)"
	@echo "TikZ   Feynman graphs dir: $(TIKZDIRNAME)"
	@echo "TikZ   Feynman graphs files: $(TIKZFILES)"


==> cover/Master_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the title page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\huge
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear
    }
  }
}


==> cover/Master_Final_Title.tex <==
%
% Title page layout for printed version
%
\titlehead{%
  \centering
  {\fontsize{44}{50}\selectfont
    Universität Bonn}

  \vspace*{20pt}

  \begin{singlespace}
    \fontsize{30}{40}\selectfont
    \InstituteName
  \end{singlespace}
}
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\vspace*{\fill}
  \raggedright
  {\normalsize
    \begin{otherlanguage}{ngerman}
      Dieser Forschungsbericht wurde als Masterarbeit von der
      Mathematisch-Naturwissenschaftlichen Fakultät der Universität Bonn
      angenommen.
    \end{otherlanguage}

    \vspace*{10ex minus 4ex}

    \noindent
    \begin{tabular}{@{}ll}
      Angenommen am:         & \thesissubmit\\
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  }
}

\maketitle


==> cover/Master_Submit_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{ngerman}
    Masterarbeit in Astrophysik\\
    angefertigt \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität\\
    Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
\lowertitleback{%
  % \begin{otherlanguage}{ngerman}
  %   Ich versichere, dass ich diese Arbeit selbstständig
  %   verfasst und keine anderen als die angegebenen Quellen und
  %   Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Datum & Unterschrift
  %   \end{tabular}
  % \end{otherlanguage}

  \begin{otherlanguage}{UKenglish}
    I hereby declare that this thesis was formulated by
    myself and that no sources or tools other than those cited were used.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Date & Signature
    \end{tabular}
  \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> thesis_cv.tex <==
\definecolor{lightgray}{gray}{0.8}
\newcolumntype{L}{>{\raggedleft}p{0.15\textwidth}}
\newcolumntype{R}{p{0.8\textwidth}}
\newcommand\VRule{\color{lightgray}\vrule width 0.5pt}

\thispagestyle{empty}
\section*{Curriculum Vitae}

\subsection*{Personal Details}

\begin{tabular}{L!{\VRule}R}
Name & Johann Schmidt \\
Date of Birth &  \\
Email & abc@physik.uni-def.de \\
Family status & Single
\end{tabular}

\subsection*{Education}

\begin{tabular}{L!{\VRule}R}
1997--2003 & Abitur, ABC Secondary School, Hamburg, Germany\\
2004--2007 & BSc in Physics, Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany.\\
2006 & CERN Summer Student, Geneva, Switzerland. \\
2007--2009 &  MSc in Physics Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany. \\
2009--2012 &  PhD in Physics, Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany. \\
2012 & Advanced Data Analysis School, Frankfurt, Germany.
\end{tabular}

\subsection*{Professional Experience}

\begin{tabular}{L!{\VRule}R}
2004 & Summer Student at CERN, Geneva, Switzerland. \\
2007--2012 & Doctoral work at the University of Bonn, Germany. \\
2008--2009 & Fieldwork at CERN, Geneva, Switzerland.\\
2011 & Talk at the Advanced Physics Conference, Timbucto
\end{tabular}

\subsection*{Languages}
\begin{tabular}{L!{\VRule}R}
German & Mother tongue \\
English & Fluent \\
Russian & Basic
\end{tabular}

